Synthetic Data Generation with Large Language Models for Personalized Community Question Answering

Personalization in Information Retrieval (IR) is a topic studied by the research community since a long time. However, there is still a lack of datasets to conduct large-scale evaluations of personalized IR; this is mainly due to the fact that collecting and curating high-quality user-related information requires significant costs and time investment. Furthermore, the creation of datasets for Personalized IR (PIR) tasks is affected by both privacy concerns and the need for accurate user-related data, which are often not publicly available. Recently, researchers have started to explore the use of Large Language Models (LLMs) to generate synthetic datasets, which is a possible solution to generate data for low-resource tasks. In this paper, we investigate the potential of Large Language Models (LLMs) for generating synthetic documents to train an IR system for a Personalized Community Question Answering task. To study the effectiveness of IR models fine-tuned on LLM-generated data, we introduce a new dataset, named Sy-SE-PQA. We build Sy-SE-PQA based on an existing dataset, SE-PQA, which consists of questions and answers posted on the popular StackExchange communities. Starting from questions in SE-PQA, we generate synthetic answers using different prompt techniques and LLMs. Our findings suggest that LLMs have high potential in generating data tailored to users' needs. The synthetic data can replace human-written training data, even if the generated data may contain incorrect information.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> latex/answer_retrieval_results_base.tex <==
\begin{table}
    \centering
    \caption{Results on SE-PQA using body context.% The symbol * indicates a statistically significant improvement over the respective non-personalized method.
    }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llccccc}
        % \toprule
        Training & Model & P@1 & NDCG@3 & NDCG@10 & MAP@100 & $\lambda$\\
        \midrule
        % \multicolumn{7}{l}{\textit{Best Answer}}\\ 
        - & BM25 &  0.279 & 0.353 & 0.394 &  0.362 & -\\
        
        \midrule
        
        \multirow{2}{*}{\textit{Best Answer}}
        & DistilBERT &  0.253 & 0.329 & 0.378 &  0.344 & -\\
        & BM25 + DistilBERT & 0.333* & 0.415* & 0.456* &  0.421* & .3\\
        
        % & MiniLM &  0.211 & 0.281 & 0.331 &  0.297 & -\\
        % & BM25 + MiniLM & 0.317* & 0.395* & 0.436* &  0.402* & .3\\
        \midrule
        % \multicolumn{7}{l}{\textit{Phi-mini}}\\
        % \midrule
        \multirow{2}{*}{\textit{Phi-mini}}
        
        & DistilBERT &  0.294* & 0.369* & 0.413* &  0.379* & -\\
        & BM25 + DistilBERT & 0.342* & 0.425* & 0.464* &  0.429* & .3\\

        % & MiniLM &  0.224 & 0.291 & 0.338 &  0.307 & -\\
        % & BM25 + MiniLM & 0.311* & 0.390* & 0.431* &  0.397* & .4\\
        
        \midrule
        % \multicolumn{7}{c}{\textit{Phi-medium}}\\ 
        % \hline
        \multirow{2}{*}{\textit{Phi-medium}}
        
        & DistilBERT &  0.301* & 0.375* & 0.419* &  0.385* & -\\
        & BM25 + DistilBERT & 0.338* & 0.423* & 0.463* &  0.427* & .4\\
        
        % & MiniLM &  0.231 & 0.298 & 0.345 &  0.313 & -\\
        % & BM25 + MiniLM & 0.312* & 0.392* & 0.433* &  0.399* & .4\\
        
        \midrule
        % \multicolumn{7}{c}{\textit{GPT-3.5}}\\ 
        % \hline
        \multirow{2}{*}{\textit{GPT-3.5}}
        & DistilBERT &  0. & 0. & 0. &  0. & -\\
        & BM25 + DistilBERT & 0. & 0. & 0. &  0. & .3\\

        % & MiniLM &  0. & 0. & 0. &  0. & -\\
        % & BM25 + MiniLM & 0. & 0. & 0. &  0. & .3\\
        
    \end{tabular}
    }
    \label{tab:answer_body_context}
    
    \caption{Results on SE-PQA with body base. %The symbol * indicates a statistically significant improvement over the respective non-personalized method.
    }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llccccc}
        % \toprule
        Training & Model & P@1 & NDCG@3 & NDCG@10 & MAP@100 & $\lambda$\\
        
        \midrule
        
        \multirow{2}{*}{\textit{Phi-mini}}
        
        & DistilBERT &  0.264* & 0.340* & 0.388* &  0.352* & -\\
        & BM25 + DistilBERT & 0.336* & 0.419* & 0.460* &  0.425* & .3\\

        % & MiniLM &  0.225 & 0.291 & 0.338 &  0.307 & -\\
        % & BM25 + MiniLM & 0.312* & 0.390* & 0.432* &  0.398* & .4\\
        
        \midrule
        % \multicolumn{7}{c}{\textit{Phi-medium}}\\ 
        % \hline
        \multirow{2}{*}{\textit{Phi-medium}}
        
        & DistilBERT &  0.299* & 0.373* & 0.418* &  0.383* & -\\
        & BM25 + DistilBERT & 0.344* & 0.425* & 0.465* &  0.430* & .3\\
        
        % & MiniLM &  0.227 & 0.296 & 0.343 &  0.311 & -\\
        % & BM25 + MiniLM & 0.313* & 0.392* & 0.433* &  0.399* & .4\\
        
        \midrule
        % \multicolumn{7}{c}{\textit{GPT-3.5}}\\ 
        % \hline
        \multirow{2}{*}{\textit{GPT-3.5}}
        & DistilBERT &  0.264 & 0.335 & 0.382 &  0.348 & -\\
        & BM25 + DistilBERT & 0.326 & 0.407 & 0.447 &  0.413 & .4\\

        % & MiniLM &  0. & 0. & 0. &  0. & -\\
        % & BM25 + MiniLM & 0. & 0. & 0. &  0. & .4\\
        
    \end{tabular}
    }
    \label{tab:answer_body_base}
\end{table}

==> latex/answer_retrieval_results_pers.tex <==
\begin{table}
    \centering
    \caption{Results on SE-PQA with body personalized.% The symbol * indicates a statistically significant improvement over the respective non-personalized method.
    }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llccccc}
        
        Training & Model & P@1 & NDCG@3 & NDCG@10 & MAP@100 & $\lambda$\\
        
        \midrule
        
        \multirow{2}{*}{\textit{Phi-mini}}
        
        & DistilBERT &  0.299* & 0.374* & 0.418* &  0.384* & -\\
        & BM25 + DistilBERT & 0.345* & 0.426* & 0.465* &  0.431* & .3\\

        % & MiniLM &  0.220 & 0.287 & 0.334 &  0.303 & -\\
        % & BM25 + MiniLM & 0.312* & 0.390* & 0.432* &  0.398* & .4\\
        
        \midrule
        % \multicolumn{7}{c}{\textit{Phi-medium}}\\ 
        % \hline
        \multirow{2}{*}{\textit{Phi-medium}}
        
        & DistilBERT &  0.299* & 0.374* & 0.419* &  0.384* & -\\
        & BM25 + DistilBERT & 0.347* & 0.429* & 0.468* &  0.433* & .3\\
        
        % & MiniLM &  0.230 & 0.298 & 0.345 &  0.313 & -\\
        % & BM25 + MiniLM & 0.315* & 0.394* & 0.435* &  0.401* & .4\\
        
        \midrule
        % \multicolumn{7}{c}{\textit{GPT-3.5}}\\ 
        % \hline
        \multirow{2}{*}{\textit{GPT-3.5}}
        & DistilBERT &  0.256 & 0.327 & 0.372 &  0.340 & -\\
        & BM25 + DistilBERT & 0.324 & 0.404 & 0.445 &  0.410 & .4\\

        % & MiniLM &  0. & 0. & 0. &  0. & -\\
        % & BM25 + MiniLM & 0. & 0. & 0. &  0. & .3\\
        
    \end{tabular}
    }
    \label{tab:answer_body_pers}
    
    % \caption{Results on SE-PQA only title pers. %The symbol * indicates a statistically significant improvement over the respective non-personalized method.
    % }
    % \resizebox{\linewidth}{!}{
    % \begin{tabular}{llccccc}
        
    %     Training & Model & P@1 & NDCG@3 & NDCG@10 & MAP@100 & $\lambda$\\
        
    %     \midrule
        
    %     \multirow{2}{*}{\textit{Phi-mini}}
        
    %     & DistilBERT &  0.182 & 0.236 & 0.280 &  0.255 & -\\
    %     & BM25 + DistilBERT & 0.303* & 0.380* & 0.423* &  0.389* & .5\\

    %     % & MiniLM &  0.151 & 0.200 & 0.241 &  0.220 & -\\
    %     % & BM25 + MiniLM & 0.295* & 0.371* & 0.413* &  0.380* & .5\\
        
    %     \midrule
    %     % \multicolumn{7}{c}{\textit{Phi-medium}}\\ 
    %     % \hline
    %     \multirow{2}{*}{\textit{Phi-medium}}
        
    %     & DistilBERT &  0.176 & 0.228 & 0.271 &  0.247 & -\\
    %     & BM25 + DistilBERT & 0.302* & 0.378* & 0.421* &  0.388* & .6\\
        
    %     % & MiniLM &  0.149 & 0.198 & 0.240 &  0.218 & -\\
    %     % & BM25 + MiniLM & 0.295* & 0.371* & 0.412* &  0.379* & .6\\
        
    %     \midrule
    %     % \multicolumn{7}{c}{\textit{GPT-3.5}}\\ 
    %     % \hline
    %     \multirow{2}{*}{\textit{GPT-3.5}}
    %     & DistilBERT &  0. & 0. & 0. &  0. & -\\
    %     & BM25 + DistilBERT & 0. & 0. & 0. &  0. & .3\\

    %     % & MiniLM &  0. & 0. & 0. &  0. & -\\
    %     % & BM25 + MiniLM & 0. & 0. & 0. &  0. & .3\\
        
    % \end{tabular}
    % }
    % \label{tab:answer_pers_title}
\end{table}


% 

==> latex/confronto_tabella_history.tex <==
\begin{table}[h]
    \centering
    \caption{Example of hallucinations in the History community
    % The symbol * indicates a statistically significant improvement over the respective non-personalized method.
    }
    \resizebox{\textwidth}{!}{
\begin{tabular}{llp{.9\textwidth}}
%\multicolumn{3}{c}{Question Title} 
%Question &
%\multicolumn{2}{c}{In which book did Poirot find a four-foot long clue?}                                            \\ \hline
Question Title & \multicolumn{2}{c}{Which figure is this a statue of?}           \\ \hline
Question Body & 
 \multicolumn{2}{c}{In Ocean's 12, [...] we see this statue in the foreground. My question is, what is this statue or rather or who is this a statue of? [...] %This is not a movie question but rather a question regarding a piece of art of classical antiquity. That's why I am posting it here hoping the history buffs can help me instead of the Stack Exchange Movies Beta.
 }        \\ \hline
%\multicolumn{3}{c}{Answers}                                                  %                \\ \hline
Model & Prompt type & Answer \\ \hline
Human written &  &  It is probably a statue of \textbf{Antinous. (Or Hermes)}. In fact it is probably this one here (notice the object behind his leg). It is located in the Capitoline musuem in Rome. It is supposed to be Antinous in the shape of the Greek god Hermes.    \\ \hline
{\multirow{4}{*}{GPT 3.5}}     %& Title pers. &   I'm sorry, but I need more context to provide an accurate answer. Could you please specify which statue you are referring to? Once I have that information, I can search for relevant details about the statue's origin, location, and historical significance.             \\  
      & Body pers.          &   The statue in question is a depiction of \textbf{Laocoon and His Sons}. It is a marble sculpture from the Hellenistic period of ancient Greece and is now on display at the Vatican Museums in Rome. [...] \\
      %The sculpture represents the Trojan priest Laocoon and his two sons being attacked by sea serpents. It is considered to be one of the most important examples of Hellenistic art and has been admired for its emotional intensity and dramatic realism. It has inspired numerous works of art, including a famous painting by El Greco and a reference in the novel \"Do Androids Dream of Electric Sheep?\" by Philip K. Dick.",  \\ 
  & Body base           &   The statue in Ocean's 12 that you are referring to is of the Greek goddess \textbf{Artemis}, also known as Diana in Roman mythology. [...]
  %Artemis was the goddess of the hunt, wilderness, childbirth, virginity, and fertility. The statue depicts her holding a bow and arrow, and wearing a billowing robe. The original statue was created by a sculptor named Leochares in the 4th century BC, but the one used in the film is a replica  
  \\   
      & Body context            &     The statue seen in the movie Ocean's 12 is a depiction of the ancient Greek mythological figure, \textbf{Laocoon}. He was a Trojan priest who warned his people against accepting the wooden horse from the Greeks during the Trojan War. [...]  \\ \hline


      {\multirow{4}{*}{Phi-mini}}     %& Title pers.   &  The question does not provide a description or image of the statue in question. However, considering the interests mentioned, if the statue were related to the United States, it could potentially be a figure from American history. [...]
      %If it were connected to the Baroque period, it might be a European figure from that era. Since the interests also include \"do-androids-dream-of-electric-sheep\" and \"short-stories,\" it seems there might be a mix-up in the interests provided. Nevertheless, if we focus on the United States and history, a notable statue that comes to mind is the Statue of Liberty, which represents Libertas, the Roman goddess of freedom. However, without a specific description or image, it's challenging to accurately identify the statue in question."       &  
      %\\  
      & Body pers.          &      The statue you are referring to in the Ocean's 12 scene is likely a representation of the Greek goddess \textbf{Athena}. [...] 
      %Athena is a prominent figure in Greek mythology, known for her wisdom, courage, and strategic warfare skills. She is often depicted wearing a helmet and carrying a shield, which aligns with the classical Greek aesthetic you mentioned.
      %Athena was born from the head of her father, Zeus, after he swallowed her pregnant mother, Metis. She is the goddess of wisdom, courage, inspiration, civilization, law and justice, strategic warfare, mathematics, strength, strategy, the arts, crafts, and skill. Athena is also associated with the city of Athens, which was named after her.\n\nIn the movie Ocean's 12, the statue of Athena could be used as a symbolic representation of the cunning and strategic nature of the characters, particularly Night Fox, who is known for his cleverness and resourcefulness. The statue's presence in the scene adds to the overall atmosphere and theme of the movie.\n\nWhile the statue in the movie may not be an exact replica of a specific historical artifact, it is likely inspired by the classical Greek style and the iconic image of Athena. If you are interested in exploring more about Athena and her depictions in art, you may want to look into ancient Greek sculptures and artworks, such as the famous Athena Parthenos statue by Phidias or the Athena Nike statue on the Acropolis in Athens."
      \\ 
  & Body base           & The statue you're referring to in the Ocean's 12 scene is likely a representation of the Greek goddess \textbf{Athena}. [...] 
  %Athena is a prominent figure in Greek mythology, known as the goddess of wisdom, courage, inspiration, civilization, law and justice, strategic warfare, mathematics, strength, strategy, the arts, crafts, and skill.
  %Athena is often depicted wearing a helmet and armor, carrying a shield, and holding a spear or a shield. She is also associated with the owl, which symbolizes wisdom. The statue you saw in the movie might have been a generic representation of Athena, as she is a widely recognized figure in classical Greek art and mythology.\n\nIn the movie, the statue's presence in the scene could be a nod to the importance of wisdom and strategy, which are qualities associated with Athena. However, without a specific image or more details, it's difficult to identify the exact statue or its artist. Nonetheless, the statue's resemblance to Athena is a reasonable assumption given its classical Greek appearance and the goddess's prominence in Greek mythology."
  \\   
      & Body context            &    The statue you're referring to in "Ocean's 12" is likely a representation of the Greek goddess \textbf{Athena}. [...]
      %Athena is a prominent figure in Greek mythology, known as the goddess of wisdom, courage, inspiration, civilization, law and justice, strategic warfare, mathematics, strength, strategy, the arts, crafts, and skill.
      %In the movie, the statue is shown in the museum scene where Night Fox (played by Elliott Gould) is attempting to steal the fake coronation egg. The statue's presence in the scene adds a sense of grandeur and classical beauty, which aligns with the aesthetic of Greek mythology and its statues.\n\nAthena's statues are often depicted wearing a helmet and carrying a shield, which could be the reason for the statue's haunting appearance in the movie. The statue's presence in the scene may have been chosen to evoke a sense of ancient wisdom and power, as Athena is a symbol of these qualities.\n\nWhile it's difficult to determine the exact statue without seeing it, the description of the figure and its association with Greek mythology strongly suggests that it is a representation of Athena."
      \\ \hline
      {\multirow{4}{*}{Phi-medium}}     
      & Body pers.          &      The statue in the movie Ocean's 12 is a representation of the Greek mythological figure \textbf{Medusa}. [...] 
      %Athena is a prominent figure in Greek mythology, known for her wisdom, courage, and strategic warfare skills. She is often depicted wearing a helmet and carrying a shield, which aligns with the classical Greek aesthetic you mentioned.
      %Athena was born from the head of her father, Zeus, after he swallowed her pregnant mother, Metis. She is the goddess of wisdom, courage, inspiration, civilization, law and justice, strategic warfare, mathematics, strength, strategy, the arts, crafts, and skill. Athena is also associated with the city of Athens, which was named after her.\n\nIn the movie Ocean's 12, the statue of Athena could be used as a symbolic representation of the cunning and strategic nature of the characters, particularly Night Fox, who is known for his cleverness and resourcefulness. The statue's presence in the scene adds to the overall atmosphere and theme of the movie.\n\nWhile the statue in the movie may not be an exact replica of a specific historical artifact, it is likely inspired by the classical Greek style and the iconic image of Athena. If you are interested in exploring more about Athena and her depictions in art, you may want to look into ancient Greek sculptures and artworks, such as the famous Athena Parthenos statue by Phidias or the Athena Nike statue on the Acropolis in Athens."
      \\ 
  & Body base           &  The statue you are referring to in the movie Ocean's 12 is a representation of the Greek goddess \textbf{Aphrodite}, also known as Venus in Roman mythology. [...] 
  
  \\   
      & Body context            &    The statue you are referring to in the movie Ocean's 12 is a representation of the Greek goddess \textbf{Athena}.[...]
      
      \\ \hline
\end{tabular}
    }
    \label{tab:confronto_history}

    \end{table}

==> latex/confronto_tabella_poirot.tex <==
\begin{table*}[ht]
    \centering
    \caption{Detailed untruthful answers to the question reported in Section \ref{subsec:exploratory_analysis}. \textit{Model} and \textit{Prompt type} refer to the LLM and prompt definition we use to generate the answers.  
    %Example of hallucinations:  
    % The symbol * indicates a statistically significant improvement over the respective non-personalized method.
    }
    \resizebox{\textwidth}{!}{
\begin{tabular}{llp{\linewidth}}
% \multicolumn{3}{c}{Question Title}                                                                 \\ \hline
Question &
\multicolumn{2}{c}{In which book did Poirot find a four-foot long clue?}                                            \\ \hline
% \multicolumn{3}{c}{Answers}                                                                  \\ \hline
Model & Prompt type & Answer \\ \hline
& Real Answer  & He found it in \textbf{The Murder on the Links}, and he made that statement in \textit{Lord Edgware Dies}.        \\ \hline
      \multirow{4}{*}{GPT 3.5}
      %& Title pers.           & In the book \textbf{"One, Two, Buckle My Shoe"} by Agatha Christie, the character Hercule Poirot discovered a four-foot long clue.      \\  
      & Basic           & In Agatha Christie's book \textbf{"The Mystery of the Blue Train"}, Hercule Poirot finds a four-foot long clue.      \\   
      & Personalized          & The book in which Poirot found a four-foot long clue is \textbf{"The Labours of Hercules"} by Agatha Christie.       \\ 
      & Contextual            & The book in which Poirot found a four-foot long clue is \textbf{"The Big Four"} by Agatha Christie. [...]       \\ \hline


      \multirow{4}{*}{Phi-mini}     %& Title pers.           & The book in which Hercule Poirot found a four-foot long clue is \textbf{"Murder on the Orient Express"}. [...]  \\
      & Basic           & The four-foot long clue you're referring to is found in Agatha Christie's novel \textbf{"The Mysterious Affair at Styles"}. [...] \\   
      & Personalized          & In \textbf{"The A.B.C. Murders"} Hercule Poirot finds a four-foot long clue. [...] \\
      & Contextual            & The clue you're referring to is found in Agatha Christie's novel \textbf{"The Mysterious Affair at Styles"} However, it's important to note that the clue mentioned in the book is not exactly four feet long. [...] 
      \\ \hline
      \multirow{4}{*}{Phi-medium}     %& Title pers. & In Agatha Christie's novel \textbf{"The ABC Murders"}, Hercule Poirot finds a four-foot long clue in the form of an ABC railway guide. [...]
      %\\  
      & Basic           & In the Agatha Christie novel \textbf{"The ABC Murders"} Hercule Poirot mentions a four-foot long clue. This clue is a piece of string that Poirot finds at the scene of one of the murders. [..] 
      \\
      & Personalized & The book in which Hercule Poirot found a four-foot long clue is \textbf{"The Mystery of the Blue Train"}.
      \\ 
      
  %The string is significant because it is a part of the killer's modus operandi, as he leaves a piece of string at each crime scene. Poirot uses this clue, along with other evidence, to solve the case and apprehend the murderer."
      & Contextual            &   In the Agatha Christie novel \textbf{"The ABC Murders"} Hercule Poirot finds a four-foot long clue. This clue is a piece of string that connects the crime scenes, which Poirot uses to unravel the mystery behind the serial killings. [...]
      %The string is a significant piece of evidence that helps Poirot identify the murderer and solve the case."     
      \\ \hline
\end{tabular}
    }
    \label{tab:confronto_Poirot}

    \end{table*}
